GAR-meets-RAG Paradigm for Zero-Shot Information Retrieval

Given a query and a document corpus, the information retrieval (IR) task is to output a ranked list of relevant documents. Combining large language models (LLMs) with embedding-based retrieval models, recent work shows promising results on the zero-shot retrieval problem, i.e., no access to labeled data from the target domain. Two such popular paradigms are generation-augmented retrieval or GAR (generate additional context for the query and then retrieve), and retrieval-augmented generation or RAG (retrieve relevant documents as context and then generate answers). The success of these paradigms hinges on (i) high-recall retrieval models, which are difficult to obtain in the zero-shot setting, and (ii) high-precision (re-)ranking models which typically need a good initialization. In this work, we propose a novel GAR-meets-RAG recurrence formulation that overcomes the challenges of existing paradigms. Our method iteratively improves retrieval (via GAR) and rewrite (via RAG) stages in the zero-shot setting. A key design principle is that the rewrite-retrieval stages improve the recall of the system and a final re-ranking stage improves the precision. We conduct extensive experiments on zero-shot passage retrieval benchmarks, BEIR and TREC-DL. Our method establishes a new state-of-the-art in the BEIR benchmark, outperforming previous best results in Recall@100 and nDCG@10 metrics on 6 out of 8 datasets, with up to 17% relative gains over the previous best.

==> 5.7-table_tydi.tex <==
\subsection{Results on \mrtydi}

% Mr. TyDI results
\begin{table}
\caption{Results (\ndcg@10) on \mrtydi dataset (\cite{mrtydi})}
\label{tab:mrtydi}
\resizebox{1\columnwidth}{!}{%
\centering
\begin{tabular}{c c c c c c c}
    \toprule
    Language & \bm & \mmarco \cite{mmarco} & \rankgpt & \rrr (this work) \\
    \toprule
    Arabic  & 0.392 & 0.682 & 0.726 & \\
    Bengali  & 0.456 & 0.660 & 0.644 & \\
    Finnish  & 0.299 & 0.541 & 0.623 & \\
    Indonesian  & 0.518 & 0.699 & 0.755 & \\ 
    Japanese  & 0.274 & 0.498 & 0.582 & \\
    Korean  & 0.263 & 0.440 & 0.496 & \\
    Russian  & 0.340 & 0.532 & 0.534 & \\
    Swahili  & 0.452 & 0.603 & 0.677 & \\
    Telugu  & 0.370 & 0.689 & 0.622 & \\
    Thai  & 0.446 & 0.684 & 0.634 & \\
    \toprule
    Avg  & 0.381 & 0.603 & 0.629 & \\
    \toprule
\end{tabular}
}
\end{table}

==> 8-checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% \textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [\textbf{Yes}/No/Not Applicable]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [\textbf{Yes}/No/Not Applicable]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [\textbf{Yes}/No/Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes/No/\textbf{Not Applicable}]
   \item Complete proofs of all theoretical results. [Yes/No/\textbf{Not Applicable}]
   \item Clear explanations of any assumptions. [Yes/No/\textbf{Not Applicable}]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [\textbf{Yes}/No/Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [\textbf{Yes}/No/Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [\textbf{Yes}/No/Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [\textbf{Yes}/No/Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [\textbf{Yes}/No/Not Applicable]
   \item The license information of the assets, if applicable. [\textbf{Yes}/No/Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes/No/\textbf{Not Applicable}]
   \item Information about consent from data providers/curators. [Yes/No/\textbf{Not Applicable}]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Yes/No/\textbf{Not Applicable}]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Yes/No/\textbf{Not Applicable}]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Yes/No/\textbf{Not Applicable}]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Yes/No/\textbf{Not Applicable}]
 \end{enumerate}

 \end{enumerate}

==> Tikz_Figures/rrr_intro.tex <==
\newcommand{\mx}[1]{\mathbf{\bm{#1}}} % Matrix command
\newcommand{\vc}[1]{\mathbf{\bm{#1}}} % Vector command

% Define the layers to draw the diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define block styles used later

\tikzstyle{sensor}=[draw, fill=blue!20, text width=5em, 
    text centered, minimum height=2.5em,drop shadow]
\tikzstyle{ann} = [above, text width=5em, text centered]
\tikzstyle{wa} = [sensor, text width=10em, fill=red!20, 
    minimum height=6em, rounded corners, drop shadow]
\tikzstyle{sc} = [sensor, text width=13em, fill=red!20, 
    minimum height=10em, rounded corners, drop shadow]

% Define distances for bordering
\def\blockdist{2.3}
\def\edgedist{2.5}

\begin{tikzpicture}
    \node (wa) [wa]  {System Combination};
    \path (wa.west)+(-3.2,1.5) node (asr1) [sensor] {$ASR_1$};
    \path (wa.west)+(-3.2,0.5) node (asr2)[sensor] {$ASR_2$};
    \path (wa.west)+(-3.2,-1.0) node (dots)[ann] {$\vdots$}; 
    \path (wa.west)+(-3.2,-2.0) node (asr3)[sensor] {$ASR_N$};    
   
    \path (wa.east)+(\blockdist,0) node (vote) [sensor] {$\theta_0,\theta_1,...,\theta_M$\\Estimated Parameters};

    \path [draw, ->] (asr1.east) -- node [above] {} 
        (wa.160) ;
    \path [draw, ->] (asr2.east) -- node [above] {} 
        (wa.180);
    \path [draw, ->] (asr3.east) -- node [above] {} 
        (wa.200);
    \path [draw, ->] (wa.east) -- node [above] {} 
        (vote.west);

               
    \path (wa.south) +(0,-\blockdist) node (asrs) {System Combination - Training};
  
    \begin{pgfonlayer}{background}
        \path (asr1.west |- asr1.north)+(-0.5,0.3) node (a) {};
        \path (wa.south -| wa.east)+(+0.5,-0.3) node (b) {};
        \path (vote.east |- asrs.east)+(+0.5,-0.5) node (c) {};
          
        \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
            (a) rectangle (c);           
        \path (asr1.north west)+(-0.2,0.2) node (a) {};
            
    \end{pgfonlayer}
    
    % Validation Layer is the same except that there are a set of nodes and links which are added
   

    \path (wa.south)+(-2.0,-7.5) node (syscomb) [sc] {\textbf{System Combination \\Algorithm}\\Estimated Parameters\\from training};
    \path (syscomb.west)+(-2.2,1.5) node (asrt1) [sensor] {$ASR_1$};
    \path (syscomb.west)+(-2.2,0.5) node (asrt2)[sensor] {$ASR_2$};
    \path (syscomb.west)+(-2.2,-1.0) node (dots)[ann] {$\vdots$}; 
    \path (syscomb.west)+(-2.2,-2.0) node (asrt3)[sensor] {$ASR_N$};    

    \path [draw, ->] (asrt1.east) -- node [above] {} 
        (syscomb.160) ;
    \path [draw, ->] (asrt2.east) -- node [above] {} 
        (syscomb.180);
    \path [draw, ->] (asrt3.east) -- node [above] {} 
        (syscomb.200);

               
    \path (wa.south) +(0,-\blockdist) node (sct) {System Combination - Training};
 

    \path (syscomb.east)+(1.0,0.0) node (bwtn) {};

    % Note how the single nodes are repeated using for loop
    \foreach \x in {0,1,...,4} 
    { 
        \draw (bwtn.east)+(\x,0) node (asr\x-2)[]{}; 
        \fill (bwtn.east)+(\x,0) circle (0.1cm); 
    }
   
    \path [draw, ->] (syscomb.east) -- node [above] {} 
        (bwtn.east);
	\path [draw, ->] (asr0-2) -- node [above] {@} 
        (asr1-2);
    \path [draw, -] (asr1-2) -- node [above] {b} 
        (asr2-2);
    \path [draw, -] (asr2-2) -- node [above] {z} 
        (asr3-2);
    \path [draw, -] (asr3-2) -- node [above] {} 
        (asr4-2);

    \path [draw, ->] (asr0-2) edge[bend  right]  node [below] {@} 
        (asr1-2);
    \path [draw, ->] (asr1-2) edge[bend  right]  node [below] {b} 
        (asr2-2);
    \path [draw, ->] (asr2-2) edge[bend  right]  node [below] {c} 
        (asr3-2);
    \path [draw, ->] (asr4-2) node[]{} (asr4-2)+(1.0,0);

    \begin{scope}[looseness=1.6]
        \path [draw, ->] (asr0-2) edge[bend  right=90]  node [below] {a} 
            (asr1-2);
        \path [draw, ->] (asr1-2) edge[bend  right=90]  node [below] {b} 
            (asr2-2);
        \path [draw, ->] (asr2-2) edge[bend  right=90]  node [below] {c} 
            (asr3-2);
    \end{scope}
    \path (asr3-2.east)+(1.5,0.0) node (bw)[sensor] {Best Word Sequence\\$\arg\max$};    

    \path [draw, -] (asr1-2.east) node [below] {} 
        (bw.west);
          
    \begin{pgfonlayer}{background}
        \path (asrt1.west)+(-0.5,1.0) node (g) {};
        \path (bw.east |- syscomb.south)+(0.5,-1.5) node (h) {};
         
        \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
            (g) rectangle (h);

        \path [draw, ->] (vote.south) edge[bend  left=90]  node [below] {Used in validation} 
            (syscomb.30);            

    \end{pgfonlayer}
    
    \path (asr1-2.south) +(-\blockdist,-\blockdist) 
        node (asrs) {System Combination - Validation};

\end{tikzpicture}
